From Duels to Battefields: Computing Equilibria of Blotto and Other Games

We study the problem of computing Nash equilibria of zero-sum games. Many natural zero-sum games have exponentially many strategies, but highly structured payoffs. For example, in the well-studied Colonel Blotto game (introduced by Borel in 1921), players must divide a pool of troops among a set of battlefields with the goal of winning (i.e., having more troops in) a majority. The Colonel Blotto game is commonly used for analyzing a wide range of applications from the U.S presidential election, to innovative technology competitions, to advertisement, to sports. However, because of the size of the strategy space, standard methods for computing equilibria of zero-sum games fail to be computationally feasible. Indeed, despite its importance, only a few solutions for special variants of the problem are known. In this paper we show how to compute equilibria of Colonel Blotto games. Moreover, our approach takes the form of a general reduction: to find a Nash equilibrium of a zero-sum game, it suffices to design a separation oracle for the strategy polytope of any bilinear game that is payoff-equivalent. We then apply this technique to obtain the first polytime algorithms for a variety of games. In addition to Colonel Blotto, we also show how to compute equilibria in an infinite-strategy variant called the General Lotto game; this involves showing how to prune the strategy space to a finite subset before applying our reduction. We also consider the class of dueling games, first introduced by Immorlica et al. (2011). We show that our approach provably extends the class of dueling games for which equilibria can be computed: we introduce a new dueling game, the matching duel, on which prior methods fail to be computationally feasible but upon which our reduction can be applied.

==> conclusion.tex <==
\section{Conclusion}
We presented polynomial time algorithms to find Nash equilibria of the well-known Colonel Blotto and General Lotto games. After many years from introducing the Colonel Blotto game by Borel, our method solves this game in a general form where the game may be asymmetric across both battlefields and players. We further showed that not only our method solves the Colonel Blotto game but it can be used as a strong tool to solve a wider range of games. 
%We studied the class of dueling games introduced by Immorlica et al. \cite{duel11} and presented a new framework which solves Poly

We introduced the class of \textit{Polynomially-separable bilinear dueling games} which is a superset of \textit{Polynomially-representable bilinear dueling games} and presented a framework to solve such games. We believe our framework provides a simple tool for solving a broad class of zero-sum games. %\textit{Polynomially-separable bilinear dueling games}.

%This means the outcome of each battlefield may be determined by any arbitrary function and players may have different number of troops. 

We also solved the classic version of the General Lotto game and showed that our method can also solve a generalized version of the problem where the payoff function is a \textit{bounded distance function}. %the game can also be solved for a variety of payoff functions called bounded distance functions.

% We further studied the dueling framework introduced by Immorlica et al. \cite{duel11}


==> ellipsoid-method.tex <==
%\section{Ellipsoid Method}

==> general-lotto.tex <==
\section{General Lotto}
\subsection{Pure strategies of General Lotto games}
Given the General Lotto game $\Gamma(a, b, f)$, player $A$ gives a probability distribution $X$ over non-negative integers such that $\mathbb{E}(X)=a$ and player $B$ gives a probability distribution $Y$ over non-negative integers such that $\mathbb{E}(Y)=b$. 

For any strategy $X$ for $A$, let $\pr{X}{i}$ be the probability that the strategy $X$ chooses $i$. By the definition we have, $\sum_{i=0}^{+\infty} {\pr{X}{i}} = 1$ and $\sum_{i=0}^{+\infty}{i\pr{X}{i}}=a$.

\begin{lemma}\label{mins}
Given a strategy $X$ with $a$ units, for any integer $x$ we have $\sum_{i=0}^x{\pr{X}{i}} \geq 1-\frac{a}{x+1}$.
\end{lemma}
\begin{proof}
We know $\sum_{i=0}^{+\infty}{i\pr{X}{i}} = a$, thus $(x+1)\sum_{i=x+1}^{+\infty}{\pr{X}{i}} \leq a$. $\sum_{i=0}^x{\pr{X}{i}}=1-\sum_{i=x+1}^{+\infty}{\pr{X}{i}}$, therefore $$\sum_{i=0}^x{\pr{X}{i}} \geq 1-\frac{a}{x+1}.$$\qed
%$\sum_{i=0}^x{\pr{X}{i}} + \sum_{i=x+1}^{+\infty}{i\pr{X}{i}} = a$.
\end{proof}
\begin{lemma}\label{maxs}
Given an NE(X, Y) for the Lotto game $\Gamma(a, b, f)$, we have $\sum_{i=0}^{b-1}{\pr{X}{i}} \leq \frac{t_f}{t_f+1}$.
\end{lemma}
\begin{proof}
Let $Y'$ be a strategy for $B$ that chooses $b-1$ with probability $p$ and chooses $b+t_f-1$ with probability $1-p$. Thus $p=\frac{t_f-1}{t_f}$. The payoff for player $B$ with strategy $Y'$ is 
\begin{equation}\nonumber
\begin{split}
&h_{\Gamma}^B(X,Y') = \sum_{i=0}^{+\infty}{\pr{X}{i}(pf(b-1, i) + (1-p)f(b+t_f-1, i))}=\\
&\sum_{i=0}^{b-1}{\pr{X}{i}(pf(b-1,i)+(1-p)f(b+t_f-1, i))} + \\
&\sum_{i=b}^{+\infty}{\pr{X}{i}(pf(b-1, i) + (1-p)f(b+t_f-1, i))}.
\end{split}
\end{equation}
Since $b\leq a$ and $X$ is in equilibrium, $h_{\Gamma}^B(a, b, f) \leq 0$. Moreover, 
\begin{equation}\nonumber
\begin{split}
&\sum_{i=0}^{b-1}{\pr{X}{i}pf(b-1, i)} \geq 0 \\ 
&\sum_{i=0}^{b-1}{\pr{X}{i}(1-p)f(b+t_f-1, i)} \geq (1-p)f_m\sum_{i=0}^{b-1}{\pr{X}{i}} \\ &\sum_{i=b}^{+\infty}{\pr{X}{i}pf(b-1, i)} \geq -pf_m\sum_{i=b}^{+\infty}{\pr{X}{i}} \\ &\sum_{i=b}^{+\infty}{\pr{X}{i}(1-p)f(b+t_f-1, i)} \geq  -(1-p)f_m\sum_{i=b}^{+\infty}{\pr{X}{i}}.
\end{split}
\end{equation}
 Therefore, 
\begin{equation}\nonumber
 (1-p)f_m\sum_{i=0}^{b-1}{\pr{X}{i}} - pf_m(1-\sum_{i=0}^{b-1}{\pr{X}{i}})-(1-	p)f_m(1-\sum_{i=0}^{b-1}{\pr{X}{i}}) \leq 0.
 \end{equation}
  Thus, $$ \sum_{i=0}^{b-1}{\pr{X}{i}} \leq \frac{1}{2-p}=\frac{t_f}{t_f+1}.$$\qed
\end{proof}

\begin{lemma}
Given an NE(X, Y) for the Lotto game $L(a, b, f)$, for any variable $x \in X$, with non-zero probability $x\leq 2(4at_f+4a)+3t_f$, and for any $y \in Y$ with non-zero probability $ y \leq 2(4at_f+4a)+2t_f$.
\end{lemma}
\begin{proof}
We first prove there is no integer $z>2(4at_f+4a)+2t_f$ in $Y$, with non-zero probability. The proof is by contradiction. Let $z> 2(4at_f+4a)+2t_f$ be an integer with non-zero probability in $Y$. By Lemma \ref{gg} there is a pair strategy $T_{x, z}^a$ with probabilities $1-p$ and $p$ in $y$. Let $y=4at_f+4a+t_f$. We consider another pair strategy $T_{x, y}^b$ with probabilities $1-q$ and $q$.
%Let $(x, z)$ be a pair in $B$ with $z>2(4at_f+4a+t_f)$ where the probability of choosing $z$ is $p$ and $x$ is $1-p$. We find another pair $x, y$ where $y=a(4t_f+4)+t_f$ with probabilities $q$ and $1-q$.
Since $Y$ is in NE, $h_{\Gamma}^Y(X, T_{x, z}^b) - h_{\Gamma}^Y(X, T_{x, y}^b) \geq 0$, so $\sum_{i=0}^{+\infty}{\pr{X}{i}((1-p)f(x, i) + pf(z, i))} - \sum_{i=0}^{+\infty}{\pr{X}{i}((1-q)f(x, i) + qf(y, i))} \geq 0$. Thus, 
\begin{equation}\label{maineq}
\begin{split}
&\sum_{i=0}^{x}{\pr{X}{i}(((1-p)f(x, i) + pf(z, i)) - ((1-q)f(x, i) + qf(y, i))) } + \\
&\sum_{i=x+1}^{+\infty}{\pr{X}{i}((1-p)f(x, i) - (1-q)f(x, i))} + \\
& - \sum_{i=x+1}^{y-t_f}{\pr{X}{i}qf(y, i)} - \sum_{i=y-t_f+1}^{+\infty}{\pr{X}{i}qf(y, i)} +\\
&\sum_{i=x+1}^{+\infty}{\pr{X}{i}pf(z, i)} \geq 0.
%&\sum_{i=x+1}^{+\infty}{\pr{X}{i}((1-p)f(x, i) + (1-q)f(x, i))} + \\
%&\sum_{i=x+1}^{y-t}{\pr{X}{i}q(1-p)f(y, i)} + \\
%&\sum_{i=y-t+1}^{+\infty}{\pr{X}{i}qf(y, i)}+\\
%&\sum_{i=x+1}^{+\infty}{\pr{X}{i}pf(z, i)} \geq 0.
\end{split}
\end{equation}
Since $y, z \geq x+t$, $f(z, i)=f(y, i)=f_m$ for all $i \leq y-t$. $(1-p) \geq (1-q)$, thus
\begin{equation}\label{subeq1}
\begin{split}
&\sum_{i=0}^{x}{\pr{X}{i}(((1-p)f(x, i) + pf(z, i)) - ((1-q)f(x, i) + qf(y, i))) } \leq 0, \\
&\sum_{i=x+1}^{+\infty}{\pr{X}{i}((1-p)f(x, i) - (1-q)f(x, i))} \leq 0,\\
& - \sum_{i=x+1}^{y-t_f}{\pr{X}{i}qf(y, i)} = - qf_m\sum_{i=x+1}^{y-t_f}{\pr{X}{i}}.
\end{split}
\end{equation}
For any arbitrary integers $i$ and $j$, $f(i, j) \leq f_m$, thus
\begin{equation}\label{subeq2}
\begin{split}
&- \sum_{i=y-t_f+1}^{+\infty}{\pr{X}{i}qf(y, i)} \leq qf_m\sum_{i=y-t_f+1}^{+\infty}{\pr{X}{i}}, \\
&\sum_{i=x+1}^{+\infty}{\pr{X}{i}pf(z, i)} \leq pf_m\sum_{i=x+1}^{+\infty}{\pr{X}{i}}.
\end{split}
\end{equation}
Therefore by Equations \ref{maineq}, \ref{subeq1}, and \ref{subeq2}, $$-qf_m\sum_{i=x+1}^{y-t_f}{\pr{X}{i}} + qf_m\sum_{i=y-t_f+1}^{+\infty}{\pr{X}{i}} + pf_m\sum_{i=x+1}^{+\infty}{\pr{X}{i}} \geq 0.$$
$y-t=4at_f+4a$ and by Lemma \ref{mins} $\sum_{i=0}^{y-t_f}{\pr{X}{i}} \geq \frac{4t_f+3}{4t_f+4}$. By Lemma \ref{maxs} $\sum_{i=0}^{x} \leq \frac{t_f}{t_f+1}$, thus $\sum_{i=x+1}^{y-t_f}{\pr{X}{i}} \geq 3\sum_{i=y-t_f}^{+\infty}{\pr{X}{i}}$, and thus $\frac{p}{q} \geq \frac{1}{2}$, thus $z \leq 2y$, which is a contradiction. Moreover, by the definition of $f$ there is no variable with non-zero probability in $X$, greater than $2(4at_f+4a)+3t_f$.\qed
\end{proof}

%For a general class of evaluation functions $f$, we prove that $\Gamma(a, b, f)$ has an NE and give a polynomial time algorithm to find such NE. Now we consider some useful properties for the payoff function $f$.
%\begin{itemize}
%\item $f$ is symmetric, which means $f(x)=-f(-x)$.
%\item $f$ is non-decreasing.
%\item There is a point $t_f$ in which $f$ becomes stable, which means $f(x\geq t)=f(t)$.
%\end{itemize}
%$All the considered properties for $f$ are obviously reasonable. In the simple lotto game we have:
%\begin{equation}\nonumber
%f(x)=
%\begin{cases}
%1 & x > 0 \\
%0 & x=0\\
%-1 & x<0
%\end{cases}
%\end{equation}


==> lotto.tex <==

\section{Generalizing Blotto Games: Colonel Lotto and General Lotto}
\label{sec:results.lotto}

In each of the examples described thus far, the zero-sum game being considered has a finite set of strategies.   In this section we demonstrate an application of our techniques to a game with infinitely many pure strategies.  We begin by describing the Colonel Lotto game, which has finitely many strategies, and then proceeding to the infinite-strategy variant: General Lotto.

\medskip

\noindent \textbf{Colonel Lotto.} The Colonel Lotto game is a variant of the Colonel Blotto game. In the Colonel Lotto game,  a pure strategy of each player  is a partition of troops into $k$ corps. Let $\px$ and $\py$ be pure strategies of players $A$ and $B$, respectively.
One corps from each side is chosen uniformly at random and the chosen corps determine the outcome of the game. 
The payoff of players $A$ and $B$ are $u^A(x_i, y_j)$ and $u^B(x_i, y_j)$ respectively, where $i$ and $j$ are the chosen corps of players $A$ and $B$.
The overall payoff of the Colonel Lotto game for players $A$ and $B$ is $h_{\mathcal{L}}^A(\px, \py) = \frac{1}{k^2}\sum_i \sum_j u^A(x_i, y_i)$ and $h_{\mathcal{L}}^B(\px, \py) = - h_{\mathcal{L}}^A(\px, \py)$ respectively.

Hart \cite{H07} proved that each Colonel Lotto game is a special case of a Colonel Blotto game in which all payoff functions are the same, i.e., for all corps $i$, we have $u^A_i() = u^A()$ and $u^B_i() = u^B()$. Therefore, we can conclude the following results based on Theorem \ref{thm:blotto}.
\begin{corollary*}
There is a polynomial-time algorithm which finds an equilibrium of any Colonel Lotto game.
\end{corollary*}

\medskip

\noindent \textbf{General Lotto.} 
The General Lotto game is a relaxation of the Colonel Lotto game (See \cite{H07} for details). In this game each player's strategy is a distribution of a nonnegative integer-valued random variable with a given expectation. In particular, players $A$ and $B$ simultaneously determine (two distributions of) two nonnegative integer-valued random variables $X$ and $Y$, respectively, such that $\E[X]=a$ and $\E[Y]=b$. The payoff of player $A$ is 
\begin{eqnarray}
\label{general_h}
h^A_{\Gamma}(X,Y) = \sum_{i=0}^{\infty} \sum_{j=0}^{\infty} \Pr(X=i) \Pr(Y=j)u(i,j),
\end{eqnarray}
and again the payoff of player $B$ is the negative of the payoff of player $A$, i.e., $h^B_{\Gamma}(X,Y) = -h^A_{\Gamma}(X,Y)$.
Hart \cite{H07} presents a solution for the General Lotto game when $u(i,j) = \sign(i-j)$.
%\footnote{Note that $\sign(i-j) = \begin{cases}1 & \mbox{if } i>j\\ -1 & \mbox{if } i<j\\ 0 & \mbox{if } i=j\end{cases} $}. 
Here, we generalize this result and present a polynomial-time algorithm for finding an equilibrium when $u$ is a {\em \distance\ function}. Function $u$ is a {\em \distance\ function}, if one can write it as $u(i,j) = f_u(i-j)$ such that $f_u$ is a monotone function and reaches its maximum value at $\um = f_u(\ut)$ where $\ut \in O(\poly(a,b))$. Note that $u(i,j)=\sign(i-j)$ is a \distance\ function where it reaches its maximum value at $i-j=1$. Now, we are ready to present our main result regarding the General Lotto game. 
\begin{theorem*} %[Theorem \ref{thm:dist}]
%\label{thm:Generallotto}
There is a polynomial-time algorithm which finds an equilibrium of a General Lotto game where the payoff function is a \distance\ function.
\end{theorem*}
\noindent \textbf{Main challenge.}
Note that in the General Lotto game, each player has infinite number of pure strategies, and thus one cannot use neither our proposed algorithm for the Colonel Blotto game nor the technique of \cite{duel11} for solving the problem. We should prune strategies such that the problem becomes tractable. Therefore, we characterize the extreme point of the polytope of all strategies, and use this characterization for pruning possible strategies.
%
To the best of our knowledge, our algorithm is the first algorithm of this kind which computes an NE of a game with infinite number of pure strategies.
%
Here, we briefly describe the proof. The complete proof is in Appendix \ref{sec:lotto}.

\noindent \textit{Step 1: Defining Finite General Lotto.}
We first solve a finite version of the problem. In the finite General Lotto game, we put a restriction on random variables and assume $X$ and $Y$ accept non-zero values only on polynomial-size sets $\D_A$ and $\D_B$ respectively.  Since the General Lotto game is a zero-sum game, a pair of strategies $(X^*, Y^*)$ is an equilibrium where $X^*$ and $Y^*$ are strategies maximizing the guaranteed payoff of player $A$ and player $B$ respectively. The following LP will find such a strategy. In particular, it finds $Pr(X=i)$, for all $i \in \D_A$, and $U$ such that: 
\begin{eqnarray}
\label{LP:5}
\max & U & \\
s.t. & \sum_{i\in \D_A} \Pr(X=i) = 1,& \nonumber\\
& \sum_{i \in \D_A} i \times \Pr(X=i) = a,& \nonumber\\
& \sum_{i \in \D_A}  \sum_{j \in \D_B} \Pr(X=i) \Pr(Y=j) u(i,j) \geq U& \forall \text{\ random\ variable\ } Y \text{\ over\ } \D_B. \label{const:5}
\end{eqnarray}
%\noindent \textit{Step 2: Characterizing extreme points (paired strategies).} 
\noindent \textit{Step 2: Computing Equilibria for Finite General Lotto.} 
A  possible pure strategy of player $B$ is a probability distribution over set $\D_B$\footnote{Note that the set of pure strategies and the set of mixed strategies are the same in this game.}. The number of constraints of LP \ref{LP:5} is therefore exponential.  However, it turns out that we can implement a separation oracle for this LP.  The finite General Lotto game is therefore polynomially separable, and hence we can compute a Nash equilibria for it by Theorem \ref{thm:bi-sep}.  We obtain the following theorem:

\begin{theorem}\label{finiteTheorem}
There is an algorithm which finds a Nash equilibrium of  finite General Lotto game in polynomial time.
\end{theorem}


%, and the problem is hard in this form. 
%We prove a structural lemma which shows it is possible to find a polynomial-size subset of pure strategies, called {\em paired strategies}, such that each pure strategy can be written as a convex combination of paired strategies (Lemma \ref{pairLemma}). In fact, paired strategies are extreme points of the polytope of all possible strategies.
%%
%In the next step, we show one of the best-response strategies of player $B$ would be a paired strategy (Lemma \ref{bslemma}).
%%
%We leverage this structural property and rewrite LP \ref{LP:5} by substituting constraints \ref{const:5} with a set of constraints over paired strategies. This reduces the size of LP and gives us the ability to solve the reduced LP and find strategy $X^*$ for the finite General Lotto game (Theorem \ref{finiteTheorem}). We use the same technique for finding strategy $Y^*$. Note that we do not need to put any restriction on payoff function $u$ for the finite General Lotto game.

\noindent \textit{Step 3: Bounding random variables.} 
At last, we analyze the General Lotto game when there is no restriction on the value of random variables $X$ and $Y$, and payoff function $u$ is a \distance \ function. We present the details of this argument in Section \ref{sec:lotto-dist} below, but first let us sketch the flow of the argument.  We first prove that the value of random variables would be bounded in any equilibrium.  To do this, we prove a structural lemma which shows it is possible to find a polynomial-size subset of pure strategies, called {\em paired strategies}, such that each pure strategy can be written as a convex combination of paired strategies (Lemma \ref{pairLemma}). In fact, paired strategies are extreme points of the polytope of all possible strategies.
%
We show one of the best-response strategies of player $B$ would be a paired strategy (Lemma \ref{bslemma}).
% It is worth mentioning that our proof heavily depends on the characterization of extreme points of the polytope of strategies which are paired strategies.
%
In particular, this structural lemma highlights the fact that the General Lotto game with a \distance \ payoff function is actually equivalent to a finite General Lotto game, and a polynomial-time algorithm characterizes its equilibrium. % (Appendix \ref{sec:distance}). 
%

\subsection{General Lotto with \distance\ functions}
\label{sec:lotto-dist}
In this section, we consider General Lotto game $\Gamma(a, b, u)$ where $u$ is a \distance\ function and design a polynomial-time algorithm for finding a Nash equilibrium of the game. 

In the following part of this section we assume $a \leq b$. Recall the definition of \distance\ functions.
%First we define the distance functions as follows.
\begin{definition}
Function $u$ is a {\distance\ function}, if one can write it as $u(i,j) = f_u(i-j)$ such that $f_u$ is a monotone function and reaches its maximum value at $\um = f_u(\ut)$ where $\ut \in O(\poly(a,b))$. We call $\ut$ the threshold of function $u$, and $\um$ the maximum of function $u$ \footnote{Note that sign function is a special case of distance functions.}.
\end{definition}

First we define a notion of paired strategies and claim that for every strategy of a player there is a best-response strategy which is a paired strategy. Then, using this observation, 
we can prove nice bounds on the set of optimal strategies.
%we design a linear program which finds an optimal strategy of each player. This results in a polynomial-time algorithm for finding a Nash equilibrium of the given finite General Lotto game.

Consider a probability distribution which only allows two possible outcomes, i.e., there are only two elements in $S$ with non-zero probabilities. We call such a distribution a \textit{paired strategy}. We define $T_{i,j}$ to be a paired strategy which only has non-zero probabilities at elements $i$ and $j$. %where $i,j\in \mathbb{N}$. 
Furthermore, we define $T_{i,j}^a$ to be a paired strategy with $\E[T_{i,j}^a]=a$. In paired strategy $T_{i,j}^a$, the probabilities of elements $i$ and $j$ are determined by $\alpha_{i,j}^a=Pr(T_{i,j}^a=i) = \frac{a-j}{i-j}$ and $\alpha_{j,i}^a = Pr(T_{i,j}^a=j)= \frac{a-i}{j-i}=1-\alpha_{i,j}^a$. In the following structural lemma, we show that every distribution $T$ over a finite set $S$ can be constructed by a set of paired strategies.
%The following theorem reveals an important structural property of General Lotto games.

\begin{lemma}\label{pairLemma}
	For every distribution $T$ over $S$ with $\E[T] = a$ and $t$ elements with non-zero probability, there are $m \leq t$ paired strategies $ \sigma_1,\sigma_2,\ldots, \sigma_m$  such that $T=\sum_{r=1}^m \beta_r \sigma_r$\footnote{This lemma claims that the strategy of a player in the finite General Lotto game can be written as a probability distribution over paired strategies. Thus $T=\beta_1\sigma_1+\beta_2\sigma_2+\ldots+\beta_m\sigma_m$ describes a strategy in which the paired strategy $\sigma_i$ is played with probability $\beta_i$.}, and for all $1 \leq i \leq m$ we have $\beta_i\in[0,1]$ and $\E[\sigma_i]=a$.
\end{lemma}
\begin{proof}
	We prove this claim by induction on the number of elements with non-zero probabilities in $T$. If there is only one element with non-zero probability  in $T$, i.e., $t=1$, then we have $Pr(T=a)=1$. Thus $T=T_{0,a}^a$ is a paired strategy and the claim holds by setting $\sigma_1=T_{0,a}^a$ and $\beta_1=1$.
	%We present a constructive proof. Consider a distribution $T$ with $\mathbb{E}(T)=a$. If $Pr(T=a) = 1$, then $T=T_{0,a}^a$ is a paired strategy and the claim is correct (let $\sigma_1=T_{0,a}^a$ and $\beta_1=1$).
	Now assuming the claim holds for all $1\leq t'< t$, we prove the claim also holds for $t$. Suppose $T$ be a probability distribution with $t$ non-zero probability elements. Since $t\geq 2$, there should be some $i<a$ with $Pr(T=i)>0$ and some $j>a$ with $Pr(T=j)>0$. We choose the largest possible number $0<\beta\leq 1$ such that $\beta \alpha_{i,j}^a\leq Pr(T=i)$ and $\beta \alpha_{j,i}^a\leq Pr(T=j)$. If $\beta = 1$, then $Pr(T=i)+Pr(T=j)\geq \alpha_{i,j}^a + \alpha_{j,i}^a=1$. This means
	$T=T_{i,j}^a$ is a paired strategy and the claim holds by setting $\sigma_1=T_{i,j}^a$ and $\beta_1=1$. Otherwise, we can write $T=(1-\beta)T'+\beta T_{i,j}^a$ where $T'=\frac{T-\beta T_{i,j}^a}{1-\beta}$. Furthermore we have
	\begin{equation*}
	\E[T'] = \frac{\E[T-\beta T_{i,j}^a]}{1-\beta} =\frac{\E[T]-\beta E[T_{i,j}^a]}{1-\beta} = a.
	\end{equation*}
	We select $\beta$ such that at least one of the probabilities $Pr[T'=i]$ or $Pr[T'=j]$ becomes zero. Thus compared to $T$, the number of elements with non-zero probability in $T'$ is at least decreased by one, and by the induction hypothesis we can write $T'=\beta'_1 \sigma'_1+\beta'_2 \sigma'_2+\ldots+\beta'_{m'} \sigma'_{m'}$ where $m'\leq t-1$. Let $\beta_i=(1-\beta)\beta'_i$ and $\sigma_i=\sigma'_i$ for $1\leq i\leq m'$ and $\beta_{m'+1}=\beta$ and $\sigma_{m'+1}=T_{i,j}^a$. Now we can write $T=\beta_1 \sigma_1+\beta_2 \sigma_2+\ldots+\beta_{m'+1} \sigma_{m'+1}$ where each $\sigma_i$ is a paired strategy and $E(\sigma_i)=a$. Furthermore, $m=m'+1\leq t$ and the proof is complete. Since $t \leq |S|$, $m$ is polynomial in the size of input. Therefore paired strategies $\sigma_1,\sigma_2,\ldots,\sigma_m$ and their corresponding coefficients $\beta_1,\beta_2,\ldots,\beta_m$ can be computed in polynomial time.
	%Now consider the case where $Pr(T=a)<1$, since $\mathbb{E}(T)=a$ there should be some $i<a$ with $Pr(X=i)>0$ and some $j>a$ with $Pr(X=j)>0$. Among all such $i$s and $j$s consider the minimum $i$ and the minimum $j$ and call them $i_1$ and $j_1$. We choose the largest possible number $0<\beta\leq 1$ such that $\beta \alpha_{i_1,j_1}\leq Pr(T=i_1)$ and $\beta (1-\alpha_{i_1,j_1})\leq Pr(T=j_1)$.
	%Then, we can write $T=(1-\beta)T'+\beta T_{i_1,j_1}^a$\footnote{If $\beta<1$, let $T'=\frac{T-\beta T_{i_1,j_1}}{1-\beta}$ and otherwise let $T'=T_{0,a}^a$.} where $\mathbb{E}(T')=a$. We selected $\beta$ such that at least one of the probabilities $Pr(T'=i_1)$ or $Pr(T'=j_1)$ are zero. let $\sigma_1=T_{i_1,j_1}^a$ and $\beta_1=\beta$. if $1-\beta>0$, we do the same process for $T'$. Call the minimum elements with non-zero probabilities in $T'$ as $i_2$ and $j_2$. Since, at least the probability for one of $i_1$ and $j_1$ has become zero in $T'$, either $i_2>i_1$ or $j_2>j_1$ and hence $i_2+j_2>i_1+j_1$. We can now find a new paired strategy $T_{i_2,j_2}^a$ and $\beta'$ such that $T'=(1-\beta')T''+\beta'T_{i_2,j_2}^a$ and then let $\sigma_2=T_{i_2,j_2}^a$ and $\beta_2=(1-\beta)\beta'$. In this way, for $k>1$, we can build $\sigma_{k}$ from previous $\sigma_j$s. Thus, we can write $T$ as the weighted sum of a sequence of paired strategy.
	%
	%Consider the sequence of $i_k+j_k$. We have already shown that this sequence is strictly increasing. Furthermore, in our construction approach we never change zero probabilities. Therefore, if $S$ is finite, then in each step the number of non-zero probability elements is at least decreased by one, and therefore after at most $|S|$ steps $\sum_{i=1}^{|S|}\beta_i$ becomes $1$.
	%\qed
\end{proof}

Our next lemma shows that paired strategies capture best-responses in the General Lotto game.

\begin{lemma}\label{bslemma}
	%For each strategy $X$ of player $A$ in finite General Lotto game $\Gamma(a,b,u,S)$, there is a best-response strategy $Y$ for player $B$ such that $Y=T_{i,j}^b$ for some $i,j\in S$.
	For every strategy of player $A$ in a finite General Lotto game there is a best-response strategy of player $B$ which is a paired strategy.
\end{lemma}

\begin{proof}
	Consider finite General Lotto game $\Gamma(a,b,u,S)$, strategy $X$ of player $A$, and a best-response strategy $Z$ of player $B$. Since $Z$ is a distribution on $S$, by using Lemma~\ref{pairLemma} we can write $Z=\sum_{r=1}^m\beta_r\sigma_r$. Thus, we have $h_\Gamma^B(X,Z)=h_\Gamma^B(X, \sum_{r=1}^m\beta_r \sigma_r)$ and because of the linearity of expectation we can write $h_\Gamma^B(X,Z)=\sum_{r=1}^m\beta_r h_\Gamma^B(X,\sigma_r)$. Since $Z$ is a best-response strategy, we have:
	%\begin{equation}
	%\forall 1\leq i,j\leq m, \hspace{.22cm} h_\Gamma^B(X,\sigma_i)= %h_\Gamma^B(X,\sigma_j).
	%\end{equation}
	\begin{equation}
	\forall 1\leq r\leq m, \hspace{.22cm} h_\Gamma^B(X,\sigma_r)= h_\Gamma^B(X,Z).
	\end{equation}
	This means paired strategy $\sigma_r$, for each $1 \leq r \leq m$, is a best-response strategy of player $B$.
	%Furthermore, since $\sum_{i=1}^m \beta_i = 1$ we have $h_\Gamma^B(X,Z)=h_\Gamma^B(X,\sigma_i)$ for all $1\leq i\leq m$. Thus, for every $1\leq i \leq m$ $Y=\sigma_i$ is a best-response strategy for player $B$.
\end{proof}

%In the following lemmas, using the structural property of the best-response strategies, we show some bounds for each player's optimal strategies. 
%\begin{lemma}\label{mins}
%For any strategy $X$ with $\mathbb{E}[X]=c$ and any integer $j$ we have $\sum_{i=0}^j{\pr{X}{i}} \geq 1-\frac{c}{j+1}$.
%\end{lemma}
%\begin{proof}
%Since $\sum_{i=0}^{+\infty}{i\pr{X}{i}} = c$, we have $(j+1)\sum_{i=j+1}^{+\infty}{\pr{X}{i}} \leq c$. This implies $$\sum_{i=0}^j{\pr{X}{i}} = 1-\sum_{i=j+1}^{+\infty}{\pr{X}{i}} \geq 1-\frac{c}{j+1}.$$
%\end{proof}
%
%\begin{lemma}\label{maxs}
%Consider  Nash equilibrium $(X, Y)$ of General Lotto game $\Gamma(a, b, u)$ where $u$ is a \distance\ function with threshold $\ut$. We have $\sum_{i=0}^{a-1}{\pr{Y}{i}} \leq \frac{\ut}{\ut+1}$.
%%\xxx[Hamid]{$a-1$ or $b-1$? I think it should be $a-1$.}
%\end{lemma}
%\begin{proof}
%Let $X'$ be a pair distribution of player $A$ that chooses $a-1$ with probability $p$ and chooses $a+{\ut}-1$ with probability $1-p$. Thus $p=\frac{\ut-1}{\ut}$. The payoff of playing strategy $X'$ against $Y$ is 
%\begin{equation}\label{ineq0}
%  \begin{aligned}
%		&h_{\Gamma}^A(X',Y)=\sum_{i=0}^{+\infty}\pr{Y}{i}[pu(a-1, i) + (1-p)u(a+{\ut}-1, i)].%=\\
%%		& \sum_{i=0}^{a-1}{\pr{Y}{i}(pu(a-1, i)+(1-p)u(a+{\ut}-1, i))}+\\
%%		& \sum_{i=a}^{+\infty}{\pr{Y}{i}(pu(a-1, i) + (1-p)u(a+{\ut}-1, i))}.
%  \end{aligned}
%\end{equation}
%
%Note that by the definition of $u$, $u(i, j) \geq 0$ if and only if $i-j \geq 0$ and $u(i, j)\leq0$ if and only if $i-j \leq 0$. Furthermore, if $i-j \geq {\ut}$ then $u(i, j)={\um}$ and if $i-j \leq -{\ut}$ then $u(i, j)=-{\um}$. Therefore,
%%\begin{eqnarray}
%%\begin{aligned}
%%	&\sum_{i=0}^{a-1}{\pr{Y}{i}pu(a-1, i)} \geq      0 \\
%%	&\sum_{i=0}^{a-1}{\pr{Y}{i}(1-p)u(a+{\ut}-1, i)} \geq     (1-p){\um}\sum_{i=0}^{a-1}{\pr{Y}{i}} \\
%%	&\sum_{i=a}^{+\infty}{\pr{Y}{i}(pu(a-1, i)+(1-p)u(a+{\ut}-1, i))} \geq     -{\um}\sum_{i=a}^{+\infty}{\pr{Y}{i}}
%%\end{aligned}
%%\end{eqnarray}
%
%\begin{equation}\label{ineq1}
%  \begin{aligned}
%	&\sum_{i=0}^{a-1}{\pr{Y}{i}pu(a-1, i)} &\geq &     &0& \\
%	&\sum_{i=0}^{a-1}{\pr{Y}{i}(1-p)u(a+{\ut}-1, i)} &\geq &    &&(1-p){\um}\sum_{i=0}^{a-1}{\pr{Y}{i}} \\
%	&\sum_{i=a}^{+\infty}{\pr{Y}{i}[pu(a-1, i)+(1-p)u(a+{\ut}-1, i)]} &\geq &    &&-{\um}\sum_{i=a}^{+\infty}{\pr{Y}{i}}
%%	&\sum_{i=a}^{+\infty}{\pr{Y}{i}(1-p)u(a+{\ut}-1, i)} &\geq &    &&-(1-p){\um}\sum_{i=a}^{+\infty}{\pr{Y}{i}}
%  \end{aligned}
%\end{equation}
%
%Note that $a \leq b$ and $(X,Y)$ is a Nash equilibrium which means $h_{\Gamma}^A(X,Y) \leq 0$. This implies  $h_{\Gamma}^A(X',Y) \leq 0$. Thus, by applying  Equality \ref{ineq0} and Inequality \ref{ineq1} we have 
%\begin{equation}\nonumber
%\begin{aligned}
% 0\geq h_\Gamma^A(X',Y) \geq     (1-p){\um}\sum_{i=0}^{a-1}{\pr{Y}{i}} 
% -{\um}\sum_{i=a}^{+\infty}{\pr{Y}{i}},
%%     -p{\um}(1-\sum_{i=0}^{a-1}{\pr{Y}{i}})
%%     -(1-	p){\um}(1-\sum_{i=0}^{a-1}{\pr{Y}{i}}). 
% \end{aligned}
% \end{equation}
%which implies 
%%\begin{equation*}
%$\sum_{i=0}^{+\infty}{\pr{Y}{i}} \geq
%  (2-p)\sum_{i=0}^{a-1}{\pr{Y}{i}}$. 
%%\end{equation*}
%  Thus, $ \sum_{i=0}^{a-1}{\pr{Y}{i}} \leq \frac{1}{2-p}$. By substituting $\frac{\ut-1}{\ut}$ instead of $p$ we can conclude $\sum_{i=0}^{a-1}{\pr{Y}{i}} \leq \frac{{\ut}}{{\ut}+1}$.
%%  \qed
%\end{proof}

Finally, in the following lemma we make use of the paired-strategy characterization to provide an upper-bound for the maximum variable with non-zero probability of a player's strategy in the equilibrium.
\begin{lemma}\label{finiteLemma}
Consider a Nash equilibrium $(X, Y)$ of General Lotto game $\Gamma(a, b, u)$ where $u$ is a \distance\ function with threshold $\ut$. If $\hat{u} = (4b{\ut}+4b+{\ut})(2{\ut}+2)$, then we have $Pr(Y>\hat{u}+{\ut})=0$ and $Pr(X>\hat{u}) = 0$.
%for any variable $x$ and $y $ with non-zero probability $x\leq 2(4a{\ut}+4a)+3{\ut}$ and $ y \leq 2(4a{\ut}+4a)+2{\ut}$, where $u$ is a distance function.
\end{lemma}
%\begin{proof}
%First, we prove for any integer $z>\hat{u}$, $\pr{X}{z} = 0$. The proof is by contradiction. Let $z > \hat{u}$ be an integer with non-zero probability in $X$. Thus there is an integer $x < a$ with non-zero probability in $X$. Consider the pair distribution $T_{x, z}^a$. We define another pair distribution $T_{x, y}^a$ where $y=4b{\ut}+4b+{\ut}$. 
%
%Consider strategy $X^{\epsilon} = X - \epsilon T_{x,z}^a + \epsilon T_{x,y}^a$.
%Note that $(X, Y)$ is a Nash equilibrium of the game. This means strategy $X$ is a best response of player $A$ to strategy $Y$ of player $B$ which implies $h_{\Gamma}^A(X, Y) \geq h_{\Gamma}^A(X^{\epsilon}, Y)$. On the other hand, because of the linearity of expectation we can write 
%$$h_{\Gamma}^A(X^{\epsilon}, Y) = h_{\Gamma}^A(X, Y) - \epsilon h_{\Gamma}^A(T_{x,z}^a, Y) + \epsilon h_{\Gamma}^A(T_{x,y}^a, Y).$$
%%
%Therefore, we conclude $w=h_{\Gamma}^A(T_{x, z}^a, Y) - h_{\Gamma}^A(T_{x, y}^a, Y) \geq 0$.
%Let $p=\alpha_{z, x}^a$ and $q=\alpha_{y, x}^a$. We have
%\begin{equation*}
%\label{mneq}
%\begin{split}
%	w=\sum_{i=0}^{+\infty}{\pr{Y}{i}[(1-p)u(x, i) + pu(z, i)]}- 
%	\sum_{i=0}^{+\infty}{\pr{Y}{i}[(1-q)u(x, i) + q u(y, i)]} \geq 0.
%\end{split}
%\end{equation*}
%We write $w$ as $w = w_1+w_2-w_3-w_4+w_5$, where 
%\begin{equation}\nonumber
%	\begin{aligned}
%		w_1=&\sum_{i=0}^{x}\pr{Y}{i}[[(1-p)u(x, i) + pu(z, i)] - [(1-q)u(x, i) + qu(y, i)]],\\
%		w_2=&\sum_{i=x+1}^{+\infty}{\pr{Y}{i}[(1-p)u(x, i) - (1-q)u(x, i)]},\\
%		w_3=&\sum_{i=x+1}^{y-{\ut}-1}{\pr{Y}{i}qu(y, i)},\\
%		w_4=&\sum_{i=y-{\ut}}^{+\infty}{\pr{Y}{i}qu(y, i)},\\
%		w_5=&\sum_{i=x+1}^{+\infty}{\pr{Y}{i}pu(z, i)}.
%	\end{aligned}
%\end{equation}
%
%%Thus, 
%%\begin{equation}\label{maineq}
%%  \begin{aligned}
%%	&\sum_{i=0}^{x}\pr{Y}{i}[((1-p)u(x, i) + pu(z, i)) - ((1-q)u(x, i) + qu(y, i))] + \\
%%	&\sum_{i=x+1}^{+\infty}{\pr{Y}{i}((1-p)u(x, i) - (1-q)u(x, i))} - \sum_{i=x+1}^{y-{\ut}-1}{\pr{Y}{i}qu(y, i)} - \\ 
%%	&\sum_{i=y-{\ut}}^{+\infty}{\pr{Y}{i}qu(y, i)} + \sum_{i=x+1}^{+\infty}{\pr{Y}{i}pu(z, i)} \geq 0.
%%  \end{aligned}
%%\end{equation}
%%\label{subeq1}
%Since $1-p \geq 1-q$ and $u(z, i)=u(y, i)={\um}$ for all $i \leq x$, we can conclude $w_1 \leq 0$.
%%\begin{equation}\label{subeq1}
%%  \begin{aligned}
%%  w_1 \leq 0
%%  \end{aligned}
%%\end{equation}
%For all $i > x$, we have $u(x, i) \leq 0$, and we also know $1-p \geq 1-q$. These mean $w_2 \leq 0$.
%%Therefore
%%\begin{equation}\label{subeq1.5}
%%w_2 \leq 0
%%\end{equation}
%Since for all $i \leq y-{\ut}$ we have $u(y, i)={\um}$, we conclude
%\begin{equation}\label{subeq2}
%	%-\sum_{i=x+1}^{y-{\ut}-1}{\pr{Y}{i}qu(y, i)} \leq 
%	w_3 = q{\um}\sum_{i=x+1}^{y-{\ut}-1}{\pr{Y}{i}}
%\end{equation}
%Moreover, for any arbitrary integers $i$ and $j$, we have $-{\um} \leq u(i, j) \leq {\um}$. Thus
%\begin{equation}\label{subeq3}
%  \begin{aligned}
%-w_4 \leq q{\um}\sum_{i=y-{\ut}}^{+\infty}{\pr{Y}{i}}
%  \end{aligned}
%\end{equation}
%\begin{equation}\label{subeq4}
%w_5 \leq p{\um}\sum_{i=x+1}^{+\infty}{\pr{Y}{i}}
%\end{equation}
%Therefore by knowing $w\geq 0$, $w_1 \leq 0$, $w_2 \leq 0$, and considering Inequalities \ref{subeq2}, \ref{subeq3}, and \ref{subeq4}, we conclude
%\begin{equation}\label{eqsun1}
%\begin{split}
%{\um}(-q\sum_{i=x+1}^{y-{\ut}-1}{\pr{Y}{i}} + q\sum_{i=y-{\ut}}^{+\infty}{\pr{Y}{i}} +  p\sum_{i=x+1}^{+\infty}{\pr{Y}{i}}) \geq w \geq 0.
%\end{split}
%\end{equation}
%$y-{\ut}-1=4b{\ut}+4b-1$ and by Lemma \ref{mins}, $\sum_{i=0}^{y-{\ut}-1}{\pr{Y}{i}} \geq 1- \frac{b}{4b{\ut}+4b}=\frac{4{\ut}+3}{4{\ut}+4}$. Note that $x<a$ which means $\sum_{i=0}^{x} \pr{Y}{i} \leq \sum_{i=0}^{a-1} \pr{Y}{i}$. On the other hand, Lemma \ref{maxs} says
%$\sum_{i=0}^{a-1} \pr{Y}{i} \leq \frac{{\ut}}{{\ut}+1}$. Hence we can conclude $\sum_{i=0}^{x} \pr{Y}{i} \leq \frac{{\ut}}{{\ut}+1}$. Therefore 
%\begin{equation}\label{eqsun2}
%\sum_{i=x+1}^{y-{\ut}-1}{\pr{Y}{i}} = \sum_{i=0}^{y-{\ut}-1}{\pr{Y}{i}} - \sum_{i=0}^{x}{\pr{Y}{i}} \geq \frac{3}{4{\ut}+4}
%\end{equation}
%and 
%\begin{equation}\label{eqsun3}
%\sum_{i=y-{\ut}}^{+\infty}{\pr{Y}{i}} = 1 - \sum_{i=0}^{y-{\ut}-1}{\pr{Y}{i}} \leq \frac{1}{4{\ut}+4}.
%\end{equation}
%
%By Inequalities \ref{eqsun1}, \ref{eqsun2}, \ref{eqsun3}, and $\sum_{i=x+1}^{+\infty}{\pr{Y}{i}} \leq 1$, we have %\xxx[Hamid]{I think you have used $\sum_{i=x+1}^{+\infty}{\pr{Y}{i}} \leq \frac{1}{{\ut}+1}$ which is incorrect.}
%\begin{equation}\label{eqsun4}
%\begin{split}
%-q \frac{3}{4{\ut}+4} + q \frac{1}{4{\ut}+4} +  p \geq 0.
%\end{split}
%\end{equation}
%which implies $\frac{q}{p} \leq 2{\ut}+2$. Recalling $p = \alpha^{a}_{z,x}=\frac{a-x}{z-x}$, $q = \alpha^{a}_{y,x}=\frac{a-x}{y-x}$, and $z>y$, we can bound $\frac{z}{y}$ as follows
%%\begin{equation*}
%$\frac{z}{y} \leq \frac{z-x}{y-x}=\frac{q}{p} \leq 2{\ut}+2$.
%%\end{equation*}
%Therefore $z \leq y (2{\ut}+2)=\hat{u}$ which is a contradiction. 
%Knowing that player $A$ put zero probability on every number $z > \hat{u}$ and considering the definition of \distance\ function $u$, player $B$ will put zero probability of every number greater than $\hat{u}+{\ut}$ in any Nash equilibrium.
%%Moreover, by the definition of $u$, increasing the units difference more than ${\ut}$ does not increase the payoff, so
%%there is no variable with non-zero probability in $Y$ greater than $8b{\ut}+8b+3{\ut}$.
%%\qed
%\end{proof}

The following theorem follows immediately from Theorem \ref{finiteTheorem} and Lemma \ref{finiteLemma}.
\begin{theorem}
\label{thm:dist}
%For a given instance of General Lotto game $\Gamma(a, b, u)$ where $u$ is a distance function, 
There is a polynomial time algorithm which finds a Nash Equilibrium of the General Lotto game $\Gamma(a, b, u)$ where $u$ is a \distance\ function.
%a Nash equilibrium can be found in time $\mathcal{O}(
%{\poly}(a, b))$.
\end{theorem}
\begin{proof}
Let $\bar{u}=(4b{\ut}+4b+{\ut})(2{\ut}+2)+{\ut}$. Lemma \ref{finiteLemma} shows there is a bound on the optimal strategies in a Nash equilibrium. More precisely $Pr(Y>\bar{u})=0$, where $Y$ is a strategy of player $A$ or $B$. Thus General Lotto game $\Gamma(a, b, u)$ is equivalent to finite General Lotto game $\Gamma(a, b, f, S)$, where $S=\{1, 2, \ldots, \bar{u}\}$. By Theorem \ref{finiteTheorem}, a polynomial-time algorithm finds a Nash equilibrium of the game.
\end{proof}








\iffalse
\subsection{To Do List}
\begin{itemize}
\item I don't know why the transformation is essential. We should explain it in more details.
\item The previous paper only considered the sign function.
\item I should mention that the discrete version is the main version.
\item Example 
\item It is better to highlight the importance of our work at the beginning of the our results section.
\item How to transform a solution from the new space to the original space.
\end{itemize}
\fi


==> model.tex <==
\section{Model}
In this section we formally define the discrete Colonel Blotto, Colonel Lotto, and General Lotto games and our notations. All these problems are resource allocation games in a competitive environment, so there are two players $A$ and $B$ with two limited amounts of resources $a$ and $b$ units. Players $A$ and $B$ simultaneously distribute their resources in some way according to the model.
\subsection*{Colonel Blotto}
The Colonel Blotto game $\mathcal{B}(a, b, k, F=\langle f_1,f_2,f_3,\ldots,f_k\rangle)$ is defined as follows. There are two players $A$ and $B$ with $a$ and $b$ units and there are $k$ independent battlefields. Each player should distribute her units into these battlefields, therefore each pure strategy for $A$ is a $k$-partition $X=\langle x_1, x_2, \ldots, x_k\rangle$ and each pure strategy for $B$ is a $k$-partition $Y=\langle y_1, y_2, \ldots, y_k\rangle$, where $\sum_{i=1}^{k}{x_i}=a$ and $\sum_{i=1}^{k}{y_i}=b$. Also $F$ is the evaluation function of the battlefields. It means that $A$'s payoff in the $i$-th battlefield is $f_i(x_i, y_i)$. Since this is a zero-sum game, $f_i(x_i, y_i)=-f_i(y_i, x_i)$. (Here we are considering a generalized version of the problem. The evaluation function is commonly defined as $f_i(x_i, y_i)=sign(x_i - y_i)$\footnote{$sign(x)$ is defined as\begin{flalign*}
&sign(x)=
\begin{cases}
1 & x > 0\\
0 & x=0\\
-1 & x<0 
\end{cases}
\end{flalign*}}
.)
The payoff for $A$ in the game is $$h_{\mathcal{B}}^A(X, Y)=\sum_{i=1}^{k}{f_i(x_i, y_i)}.$$
Thus the payoff for $B$ is $h_{\mathcal{B}}^B(X, Y)=-h_{\mathcal{B}}^A(X, Y)=\sum_{i=1}^{k}{f_i(y_i, x_i)}.$\\
The mixed strategies is to be explained.
\subsection*{Colonel Lotto}
The Colonel Lotto Game is a variant of Colonel Blotto game which is symmetrized across battlefields. More precisely, in a Colonel Lotto Game $\mathcal{L}(a, b, k, f)$ there are two players $A$ and $B$ with $a$ and $b$ units. Each strategy with $x$ units is a set $X=\{x_1, x_2, \ldots, x_k\}$, such that $\sum_{i=1}^k{x_i}=x$. So player $A$ provides a strategy $X$ with $a$ units and player $B$ provides a strategy $Y$ with $b$ units. One element $x \in X$ and one element $y\in Y$ will be randomly chosen and then evaluated by the function $f(x, y)$. The payoff is the expected value of this evaluation, which is $$h_{\mathcal{L}}^A(X, Y)=\frac{1}{k^2}\sum_{i=1}^k{\sum_{j=1}^k{f(x_i, x_j)}}.$$
\subsection*{General Lotto}
A General Lotto game $\Gamma(a, b, f)$ is defined with two players $A$ and $B$ who choose two probability distribution functions $X$ and $Y$ over non-negative integer values, such that $\mathbb{E}(X)=a$ and $\mathbb{E}(Y)=b$, and $\sum_{i=0}^{+\infty}{\pr{X}{i}}=\sum_{i=0}^{+\infty}{\pr{Y}{i}}=1$, where $\pr{X}{i}$ denotes the probability of choosing $i$ in $X$. Moreover, we define an evaluation function $f$ such that $f(x, y)$ represents the payoff if $A$ has chosen $x$ and $B$ has chosen $y$. Thus the payoff for $A$ is $$h_{\Gamma}^A(X, Y)=\sum_{i=0}^{+\infty}{\sum_{j=0}^{+\infty}{\pr{X}{i}\pr{Y}{j}f(i, j)}}$$ and again $h_{\Gamma}^B(X, Y)=-h_{\Gamma}^A(X, Y)$.
%=\sum_{i=0}^{+\infty}{\sum_{j=0}^{+\infty}{\pr{X}{i}\pr{Y}{j}f(j, i)}}$. 
%In the classic version of discrete General Lotto game, $S=\mathbb{W}$ and $f(x, y)=sign(x, y)$.
